Prototypical Cross-Attention Networks for Multiple Object Tracking and Segmentation

Multiple object tracking and segmentation requires detecting, tracking, and segmenting objects belonging to a set of given classes. Most approaches only exploit the temporal dimension to address the association problem, while relying on single frame predictions for the segmentation mask itself. We propose Prototypical Cross-Attention Network (PCAN), capable of leveraging rich spatio-temporal information for online multiple object tracking and segmentation. PCAN first distills a space-time memory into a set of prototypes and then employs cross-attention to retrieve rich information from the past frames. To segment each object, PCAN adopts a prototypical appearance module to learn a set of contrastive foreground and background prototypes, which are then propagated over time. Extensive experiments demonstrate that PCAN outperforms current video instance tracking and segmentation competition winners on both Youtube-VIS and BDD100K datasets, and shows efficacy to both one-stage and two-stage segmentation frameworks. Code and video resources are available at http://vis.xyz/pub/pcan.

==> checklist.tex <==
	\section*{Checklist}
	
	\begin{enumerate}
		
		\item For all authors...
		\begin{enumerate}
			\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
			\answerYes{}
			\item Did you describe the limitations of your work?
			\answerYes{See Section~\ref{limitation}.}
			\item Did you discuss any potential negative societal impacts of your work?
			\answerYes{See Section~\ref{impact}.}
			\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
			\answerYes{}
		\end{enumerate}
		
		\item If you are including theoretical results...
		\begin{enumerate}
			\item Did you state the full set of assumptions of all theoretical results?
			\answerYes{}
			\item Did you include complete proofs of all theoretical results?
			\answerYes{See Section~\ref{methods}.}
		\end{enumerate}
		
		\item If you ran experiments...
		\begin{enumerate}
			\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{But the code and trained models will be released upon publication.}
			\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
			\answerYes{Please refer to Section~\ref{sec:setup} and supplementary material.}
			\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Following prior work in this field, error bars are not reported because it would be too computationally expensive.}
			\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to supplementary material.}
		\end{enumerate}
		
		\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
		\begin{enumerate}
			\item If your work uses existing assets, did you cite the creators?
			\answerYes{}
			\item Did you mention the license of the assets?
    \answerYes{Please refer to the supplementary material for the license and details of the employed datasets and code.}
			\item Did you include any new assets either in the supplemental material or as a URL?
			\answerNo{Code and models will be released upon publication.}
			\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Please refer to the supplementary material for more details on the datasets.}
			\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Please refer to the supplementary material for more details on the datasets.}
		\end{enumerate}
		
		\item If you used crowdsourcing or conducted research with human subjects...
		\begin{enumerate}
			\item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
			\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
			\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
		\end{enumerate}
		
	\end{enumerate}
